Let Invariant Rationale Discovery Inspire Graph Contrastive Learning

Leading graph contrastive learning (GCL) methods perform graph augmentations in two fashions: (1) randomly corrupting the anchor graph, which could cause the loss of semantic information, or (2) using domain knowledge to maintain salient features, which undermines the generalization to other domains. Taking an invariance look at GCL, we argue that a high-performing augmentation should preserve the salient semantics of anchor graphs regarding instance-discrimination. To this end, we relate GCL with invariant rationale discovery, and propose a new framework, Rationale-aware Graph Contrastive Learning (RGCL). Specifically, without supervision signals, RGCL uses a rationale generator to reveal salient features about graph instance-discrimination as the rationale, and then creates rationale-aware views for contrastive learning. This rationale-aware pre-training scheme endows the backbone model with the powerful representation ability, further facilitating the fine-tuning on downstream tasks. On MNIST-Superpixel and MUTAG datasets, visual inspections on the discovered rationales showcase that the rationale generator successfully captures the salient features (i.e. distinguishing semantic nodes in graphs). On biochemical molecule and social network benchmark datasets, the state-of-the-art performance of RGCL demonstrates the effectiveness of rationale-aware views for contrastive learning. Our codes are available at https://github.com/lsh0520/RGCL.

==> backup/2_preliminary.tex <==
\section{Preliminary}

\subsection{Graph Contrastive Learning}

SSL has been demonstrated effective across multiple machine learning domains \cite{revisit-ssl-cv, benchmark-ssl-cv, BERT, GPT-3}. 
And pre-training strategies for GNNs \cite{DGI, GNN-pretrain, GraphCL} start to emerge to improve the representation learning ability of them.
Generally speaking, pre-training strategies for GNNs fall into two categories. The first one are predictive models, which are trained to predict certain masked properties of the original graph, such as graph context \cite{GNN-pretrain}, node attributes \cite{GNN-pretrain} and edge existence \cite{GraphSAGE}. 
In the second category are contrastive learning based models, aiming at maximizing mutual information \cite{infonce} between two views, such as node-node contrast \cite{GCC}, node-graph contrast \cite{DGI} and graph-graph contrast \cite{GraphCL}.
In this paper, we mainly focus on GCL pre-training strategies.

Inspecting on prior GCL studies, these paradigms remain within the confines of a two-step backbone: (1) graph augmentation; (2) contrastive learning.

\textbf{Graph augmentation} Graph augmentation is the prerequisite and discriminative module for various GCL frameworks, which states:
\begin{equation}
    g_A \sim A(g_A|g)
\end{equation}
where $g$ is the original graph, $g_A$ is the augmented view sampled from the augmentation distribution $A(\cdot|g)$.

Primary GCL frameworks adopt random corrupting method to conduct graph augmentation. 
\cite{GRACE} proposes a hybrid scheme - GRACE for generating graph views on both structure and attribute levels.
GCC \cite{GCC} captures the universal network topological properties across multiple networks.
GraphCL \cite{GraphCL} systematically studies the impact of various combinations of random graph augmentations on multiple datasets to validate their effectiveness.
Despite showing promising performance, the intrinsic random mechanism makes them suffer from potential semantic information loss, resulting in failure of capturing informative features. 
To tackle this problem, domain knowledge is leveraged to guide graph augmentation with the purpose of preserving discriminative characteristics. 
\lsh{MICRO-Graph \cite{motif-GCL} extracts semantically meaningful motifs (\emph{e.g.,} functional groups in biochemistry molecules) to sample informative subgraphs for contrastive learning.
GraphMVP \cite{GraphMVP} performs contrastive learning by utilizing the correspondence and consistency between 2D
topological structures and 3D geometric views of biochemistry molecules.
However, the involvement of external domain knowledge (\emph{e.g.,} motifs and 3D geometric information) severely undermines the generalization performance of aforementioned MICRO-Graph and GraphMVP.}
GCA \cite{GCA} leverages node centrality to highlight important connective structures, enforcing the model to recognize underlying semantic information.
Nevertheless, its intrinsic assumption - node centrality represents saliency does not necessarily holds in domains other than social network.

\textbf{Contrastive learner} Based on views generated by graph augmentation function set $\mathcal{A}$, contrastive learning is performed between the latent representations of two augmented views of input graph and the loss function on original graph datasets $\mathcal{G}$ can be written as:
\begin{equation}
    \mathcal{L} = \mathbb{E}_{A_1,A_2 \in \mathcal{A}}\mathbb{E}_{g\in \mathcal{G}}l(f(A_1(g)),f(A_2(g)))
\end{equation}
where $f(\cdot)$ represent the encoder, $A_i (i=1,2)$ are augmentation functions from set $\mathcal{A}$ and contrastive loss function $l$ can be set as NCE \cite{PIRL}, InfoNCE \cite{infonce}, NT-Xent \cite{SimCLR} or their variants.

\subsection{Invariant Rationale Discovery}

The goal of IRD is to generate a rationale based on input $x$, denoted as $R(x)$, which is a selection of input features that account for self-discrimination. 
An ideal rationale should first satisfy the sufficiency condition - $R(x)$ is sufficient to preserve the critical information of $x$ related to prediction $y$, \emph{i.e.}
\begin{equation}
    p_y(\cdot |R(x))=p_y(\cdot |x)
\end{equation}
Moreover, according to the comprehensiveness condition of IRD, the complement of rationale $R^c(x)$ does not contain sufficient information for prediction $y$, \emph{i.e.}
\begin{equation}
    H(y|R^c(x))\ge H(y|R(x))+h
\end{equation}
for certain constant $h$.

Concretely speaking, there are two justifications of the comprehensiveness condition. 
First, it regulates the information outside the rationale so that the rationale contains all the relevant and useful information. 
Second and more importantly, comprehensiveness is promising to prevent the explanations from degeneration, where the $R(x)$ attempts to encode the self-discrimination of $x$ using trivial information.

\subsection{Invariance Look at GCL}

State-of-the-art contrastive learning (CL) methods encourage the learned representations contain no information about the data augmentation strategies in which the data is transformed, \emph{i.e.,} to be invariant to the augmentations \cite{ECL, PIRL}.   
Let $\mathcal{A}$ be a group of transformations. 
For any $A\in \mathcal{A}$, let $A(x)$ denote the function transforms an input data $x$. 
Let $f(\cdot)$ be the encoder that computes feature representation, $f(x)$. CL encourages the encoder to learn the invariant features, which states $f(A(x))=f(x)$, \emph{i.e.} the output representation, $f(x)$, does not vary with $A(\cdot)$. 
This paradigm essentially requires the transformed data $A(x)$ to preserve the semantic information in $x$.

In the field of computer vision, semantic information in the input data can be easily preserved to satisfy the invariance conditions after performing data augmentations like rotation, color distortion and Gaussian blur. 
When it comes to GCL, it’s much more challenging and still under-explored to preserve semantic information in a general GCL framework without the guidance of any prior knowledge.
This motivation is  consistent with IRD, aiming at capturing the rationale invariant to graph augmentations and distilling the causal information to the prediction from the original graph. 

Inspired by two conditions of invariance - sufficiency and comprehensiveness, we argue that an ideal graph augmentation method is supposed to (1) reveal the semantic information related and self-discriminative features in original graph to satisfy sufficiency and (2) conceal the non-informative fraction to meet the comprehensiveness condition. 
A natural way to achieve aforementioned invariance goal in GCL is to (1) discover the rationale $R(g)$ (\emph{i.e.,} a self-discriminative subset of input graph $g$) and preserve it in augmented graphs, which states 
\begin{equation}
    f(R(g)) = f(g)
\end{equation}
and (2) push apart $R(g)$ and its complement $R^c(g)=g|R(g)$ when conducting contrastive learning, \emph{i.e.}
\begin{equation}
    f(R^c(g)) \perp f(g)
\end{equation}

==> backup/3_method.tex <==
\section{Methodology}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{charts/framework.pdf}
    \vspace{-20pt}
    \caption{RGCL framework. A rationale generator identifies a discriminative subset of nodes in the original graph. Darker color indicates higher sampling probability in the rationale/complement generation distribution. Two rationales and one complement are generated according to Equation \eqref{equ:rationale-complement-distribution}. The rationale generator, shared GNN-encoder and shared projector are jointly optimized via minimizing both the sufficiency loss (\cf Equation \eqref{equ:loss-su}) and independence loss (\cf Equation \eqref{equ:loss-in}).}
    \label{fig:framework}
    \vspace{-10pt}
\end{figure*}

Inspired by IRD, we propose a new pre-training scheme, Rationale-aware Graph Contrastive Learning (RGCL), which discovers rationales garnering self-discriminative semantics and performs contrastive learning on rationale-aware views.
We next present the pipeline of RGCL: rationale-aware graph augmentation, representation learning, and contrastive learning.

\subsection{Rationale-aware Graph Augmentation}

As prior studies \cite{GraphCL} have shown that node dropping and subgraph dropping perform well as graph augmentations across different categories of graph datasets. We thus focus on identifying a subset of salient nodes with their edges as the rationale of the anchor graph.

Towards this end, we need to assess the attribution of each node to self-discrimination.
Moreover, to maintain the diversity of augmented views, it is not sagacious to model the node contribution and rationale generation in a deterministic manner.
Hence, we adopt the idea of probabilistic sampling upon an assumption:
given an anchor graph $g$, the generation of its rationale $R(g)$ follows a probability distribution $p_{R}(R(g)|g)$, which summarizes the probability of each node being salient:
\begin{gather}\label{equ:rationale-distribution}
    p(R(g)|g)=\prod_{v\in\Set{V}}p(v|g),
\end{gather}
where $v\in\Set{V}$ is a node of $g$; $p(v|g)$ denotes the probability of $v$ being included into $R(g)$, reflecting how semantically important it is. Analogously, we can define the distribution of generating the rationale's complement $R^{c}(g)$ as:
\begin{gather}\label{equ:complement-distribution}
    p(R^{c}(g)|g)=\prod_{v\in\Set{V}}(1-p(v|g)),
\end{gather}
where $1-p(v|g)$ measures how deficient node $v$ is to accomplish self-discrimination.


By sampling from distribution $p(R(g)|g)$ and $p(R^{c}(g)|g)$ separately, we establish the stochastic rationale $R(g)$ and its complement $R^{c}(g)$ as:
\begin{gather} \label{equ:rationale-complement-distribution}
    R(g)\sim p(R(g)|g),\quad R^{c}(g)\sim p(R^{c}(g)|g),
\end{gather}
where the sampling ratio $\rho$ is a hyperparameter (\eg $80\%$). Note that $R^{c}(g)$ is not the node difference between $g$ and $R(g)$, but a stochastic complement sampled from the distribution $p(R^{c}(g)|g)$.
As a result, each node within $R(g)$ (or $R^{c}(g)$) is assigned with its probability $p(v|g)$ (or $1-p(v|g)$), which illustrates how crucial (or trivial) it is to conduct self-discrimination in GCL.


We now present how to implement the foregoing process.
Here we hire a rationale generator network $r(\cdot)$ to parameterize the probability distribution function $p(\cdot|g)$, which consists of two modules, $r=r_{1}\circ r_{0}$:
\begin{gather}
    \Mat{Z}=r_{0}(g), \quad p(v|g)=r_{1}(\Mat{z}_{v}),
\end{gather}
where $r_{0}(\cdot)$ is the GNN encoder that takes the anchor graph $g$ as input and yields the $d$-dimensional representations $\Mat{Z}\in\Space{R}^{|\Set{V}|\times d}$ for all nodes;
subsequently, $r_{1}(\cdot)$ adopts a multi-layer perceptron (MLP) with two hidden layers to get node $v$'s attribution score based on its corresponding vector $\Mat{z}_{v}$ in $\Mat{Z}$. Then the softmax function is applied over all nodes' scores to obtain the normalized probability distribution.

After sampling nodes from these two distributions, we have $R(g)$ and $R^{c}(g)$, while discarding the remaining nodes.
For the rationale-augmented view $R(g)$, we then associate it with the attribution vector $\hat{\Mat{P}}\in\Space{R}^{|\Set{V}|\times 1}$, each element of which is defined as follows: 
\begin{gather}
    \hat{p}_{v}=
    \begin{cases}
        p(v|g),\quad&\text{if}~~ v\in R(g),\\
        0,\quad&\text{otherwise}.
    \end{cases}
\end{gather}
Similarly, we set the elements of another attribution vector $\hat{\Mat{P}}^{c}\in\Space{R}^{|\Set{V}|\times 1}$ for $R^{c}(g)$ as follows:
\begin{gather}
    \hat{p}^{c}_{v}=
    \begin{cases}
        1-p(v|g),\quad&\text{if}~~ v\in R^{c}(g),\\
        0,\quad&\text{otherwise}.
    \end{cases}
\end{gather}



% \subsection{Rationale-aware Graph Augmentation}

\subsection{Rationale-aware Representation Learning}

Having established the rationale-augmented view $R(g)$ with the probability vector $\hat{\Mat{P}}$, we feed them into the GNN backbone $f(\cdot)$ (\ie the target model being pre-trained) to generate the rationale-aware representation:
\begin{gather}\label{equ:rationale-representation}
    \Mat{x}=f(R(g))=\text{Pooling}(\text{GNN}(R(g))\odot\hat{\Mat{P}})),
\end{gather}
where $f(\cdot)$ is a combination of the base encoder GNN$(\cdot)$ and the pooling layer Pooling$(\cdot)$, and yields the $d'$-dimensional rationale representation $\Mat{x}$.
To be more specific, GNN$(\cdot)$ outputs $\Mat{X}\in\Space{R}^{|\Set{V}|\times d'}$ that collects the representations of nodes within $R(g)$, while setting the all-zero vectors for nodes outside $R(g)$.
Subsequently, we apply the element-wise product between $\Mat{X}$ and $\hat{\Mat{P}}$, and then employ the pooling function $\text{Pooling}(\cdot)$ to compress the node representations into the rationale representation.
Note that, when fine-tuning on downstream tasks, we disable the rationale discovery module and discard $\hat{\Mat{P}}$ in $f(\cdot)$, \ie $\Mat{x}=\text{Pooling}(\text{GNN}(g))$.

Moreover, we resort to a projection head $h(\cdot)$ to map the graph representation into another latent space where the contrastive learning in conducted, aiming to enforce mutual information between the anchor and rationale to a tighter lower bound \cite{SimCLR}.
Formally, aforementioned process is shown as:
\begin{gather}\label{equ:rationale-projection}
    \Mat{r}=h(\Mat{x})=L_{2}(\text{MLP}(\Mat{x})),
\end{gather}
where $h(\cdot)$ is instantiated by an MLP with $l_{2}$ normalized outputs.
% $\Mat{r}=h(\Mat{x})=L_{2}(\Mat{W}^{(2)}\sigma(\Mat{W}^{(1)}\Mat{x}))$
Similarly, we can get the representation and the projection of the complement-aware view $R^{c}(g)$:
\begin{gather}\label{equ:complement-representation-projection}
    \Mat{x}^{c}=f(R^{c}(g)),\quad \Mat{c}=h(\Mat{x}^{c}).
\end{gather}



\subsection{Rationale-aware Contrastive Learning}

Given the rationale-aware graph augmentations, we move on to achieving the sufficiency and independence principles (\cf Equations \eqref{equ:sufficiency-principle} and \eqref{equ:independence-principle}) in contrastive learning.

Towards this end, for an anchor graph $g$, we randomly sample two rationales from its rationale generation distribution, view them as the positive pair $(R_1(g),R_2(g))$ of $g$, and establish their projected representations $\Mat{r}_1^+$ and $\Mat{r}_2^+$ via Equation \eqref{equ:rationale-projection}.
Following the previous work \cite{SimCLR}, the rationales of other anchors are treated as the negative views of $g$, and summarized their representations into $\Set{R}^{-}=\{\Mat{r}^-\}$.
We then model the sufficiency principle as minimizing the following contrastive loss:
\begin{gather}\label{equ:loss-su}
    l_{\text{su}}(g)=-\log\frac{\exp{(\Trans{\Mat{r}_1^+}\Mat{r}_2^+/\tau)}}{\sum_{\Mat{r}^-\in\Set{R}^{-}}\exp{(\Trans{\Mat{r}_1^+}\Mat{r}^-/\tau)}},
\end{gather}
where $\tau$ is a temperature hyperparameter.
It encourages the agreement between the positive rationale-aware views of the same anchor graph, while enforcing the divergence between different anchors.
Through minimizing $l_{\text{su}}(g)$, rationale generator is required to refine the crucial information in the anchor graph about self-discrimination, which has a causal relation with semantics (\cf Equations \eqref{equ:sufficiency-principle}).


Going beyond the negative views derived from other anchors' rationales, we further sample one complement $R^{c}(g)$ from its complement generation distribution, and cast it as the additional negative views of $g$.
And we parameterize the independency principle as the minimization of the contrastive loss below:
\begin{gather}\label{equ:loss-in}
    l_{\text{in}}(g)=-\log{\frac{\exp{(\Trans{\Mat{r}_1^+}\Mat{r}_2^+/\tau)}}{\exp{(\Trans{\Mat{r}_1^+}\Mat{r}_2^+/\tau)}+\sum_{\Mat{c}\in\Set{C}}\exp{(\Trans{\Mat{r}_1^+}\Mat{c}/\tau)}}},
\end{gather}
where $\Mat{c}\in\Set{C}$ is the complement representation appearing in the minibatch data.
The minimization of $l_{\text{in}}(g)$ pushes away the representation of the complement, \ie $\Mat{c}$, from that of the rationale, \ie $\Mat{r}$, making the captured rationale stable regardless of changes in its complement, which is consistent with the independence principle in Equation \eqref{equ:independence-principle}.

% Going beyond the negative views derived from other anchors, we further sample one complement $R^{c}(g)$ from its complement generation distribution, and cast it as the additional negative views of $g$.
% As the independence principle states that self-discrimination should be stable regardless of changes in the complements conditioning on the rationale, $R_1(g)$, $R_2(g)$ should diverge from possible complements.
% To this end, we parameterize the independency principle as the minimization of the contrastive loss below:
% \lsh{
% \begin{gather}\label{equ:loss-in}
%     l_{\text{in}}(g)=-\log{\frac{\exp{(\Trans{\Mat{r}_1^+}\Mat{r}_2^+/\tau)}}{\exp{(\Trans{\Mat{r}_1^+}\Mat{r}_2^+/\tau)}+\sum_{\Mat{c}\in\Set{C}}\exp{(\Trans{\Mat{r}_1^+}\Mat{c}/\tau)}}},
% \end{gather}
% }
% where $\Mat{c}\in\Set{C}$ is the complement representation appearing in the minibatch data.
% This loss enforces $R^{c}(g)$ to regulate the information outside the rationale.

Finally, our objective function conflates these two types of losses, depicting the cooperative game between the rationale generator network $r(\cdot)$ and the target backbone model $f(\cdot)$:
\begin{gather}\label{equ:final_loss_function}
    \min_{r,f,h}\Lapl_{\text{RGCL}}=\Space{E}_{g\in\Set{G}}l_{\text{su}}(g)+\lambda\cdot l_{\text{in}}(g),
\end{gather}
where $\lambda$ is the hyperparameter to control the tradeoff between $l_{\text{su}}(g)$ and $l_{\text{in}}(g)$.
After optimization, we throw away the projection head $h(\cdot)$ for fine-tuning on downstream tasks.
It is worth mentioning that our RGCL is a backbone-agnostic self-supervised graph learning framework, which can be applicable to different backbone models. 

% \begin{figure}[t]
% \centering
% \includegraphics[width=\columnwidth]{charts/mutag_vis.pdf}
% \vspace{-20pt}
% \caption{Visualization of Mutag graphs. The first row presents the rationales labeled by chemistry experts and the second row presents those discovered by our rationale generator.}
% \label{mutag_vis}
% \end{figure}

% \begin{figure}[t]
% \centering
% \includegraphics[width=\columnwidth]{charts/mnist_superpixel.jpg}
% \vspace{-20pt}
% \caption{Visualization of MNIST-Superpixel graphs. From top to bottom are original MNIST data, MNIST-Superpixel graph and the rationale generated by the rationale generator in RGCL. The darker color indicates higher sampling probability in rationale graphs.}
% \label{superpiexel}
% \end{figure}

}

==> chapters/reference.tex <==
\section{Graph Contrastive Learning (GCL)}

\subsection{\cite{ECL}}
In the state-of-the-art self-supervised learning (SSL) pre-training produces semantically good representations by encouraging them to be invariant under meaningful transformations prescribed from human knowledge.

Human knowledge about what makes a good representation and the abundance of unlabeled data has enabled the learning of useful representations via self-supervised learning (SSL) pretext tasks.
State-of-the-art SSL methods encourage the representations not to contain information about the way the inputs are transformed, \ie to be invariant to a set manually chosen transformations.
One such method is contrastive learning, which sets up a binary classification problem to learn invariant features.
Given a set of data points (say graphs), different transformations of the same data point constitute positive examples, whereas transformations of other data points constitute the negatives.
Here, we refer to such methods as Invariant-SSL (I-SSL).

The natural question in I-SSL is to what transformations should the representations be insensitive.

The concept of insensitivity is captured by the mathematical idea of equivariance.
Let $\Set{H}$ be a group of transformations.
For any $h\in\Set{H}$, let $T_{h}(\Mat{g})$ denote the function with which $h$ transforms an input graph $\Mat{g}$.
Let $f$ be the encoder network that computes feature representation, $f(\Mat{g})$.
I-SSL encourages the property of ``invariance to $H$'', which states:
\begin{gather}
    f(T_{h}(\Mat{g})) = f(\Mat{g}),
\end{gather}
\ie the output representation, $f(\Mat{g})$, does not vary with $T_{h}$. 



\subsection{\cite{PIRL}}
The goal of self-supervised learning from graphs is to construct graph representations that are semantically meaningful via pretext tasks that are semantically meaningful for a large training set of graphs.
We argue that, semantic representations ought to be invariant under graph transformations.

I-SSL constructs graph representations that are similar to the representation of transformed versions of the same graph and different from the representations of other graphs.


Suppose we are given a graph dataset, $\Set{D}=\{\Mat{g}\}$, and a set of graph transformations, $\Set{H}$.
The set $\Set{H}$ may contain transformations such as node/edge dropping, node/edge masking, clustering/prototyping.
We aim to train a graph neural network encoder, $f$, with parameters $\theta$ that constructs graph representations $\Mat{z}=f(\Mat{g})$ that are invariant to graph transformations $h\in\Set{H}$.
We adopt an empirical risk minimization approach to learning the encoder parameters $\theta$.
Specifically, we train the encoder by minimizing the empirical risk:
\begin{gather}
    \Lapl = \Space{E}_{h\in\Set{H}}\Space{E}_{\Mat{g}\in\Set{D}}l(f(\Mat{g}),f(T_{h}(\Mat{g}))),
\end{gather}
where the function $l(\cdot,\cdot)$ is a loss that measures the similarity between two graph representations, which can be set as NCE \cite{PIRL}, InfoNCE, NT-Xent \cite{SimCLR}.
Minimization of this loss encourages the encoder $f$ to produce the same representation for graph $\Mat{g}$ as for its transformed counterpart $T_{h}(\Mat{g})$, \ie to make representation invariant under transformation $h$.


\subsection{\cite{SimCLR}}
This paper presents SimCLR: a simple framework for contrastive learning of graph representations.
We simplify recently proposed graph contrastive self-supervised learning algorithms without requiring specialized transformations.
SimCLR learns representations by maximizing agreement between differently augmented views of the same data example via a contrastive loss in the latent space.

Many I-SSL approaches have relies on heuristics to design pretext tasks, which could limit the generality of the learned representations.

Not only does SimCLR outperform previous work, but it is also simple, requiring neither specialized nor heuristics-guided transformations.

The recent renaissance of SSL began with artificially designed pretext tasks, such as node/edge dropping, node/edge masking, clustering, prototyping.
Although good results can be obtained, these pretext tasks rely on somewhat ad-hoc heuristics, which limits the generality of learned representations.




\section{Invariant Rationale Discovery (IRD)}
\subsection{\cite{DBLP:conf/emnlp/YuCZJ19}}
Selective rationalization is to identify a subset of input features relevant for prediction (set as self-discrimination in SSL).
The setup can be viewed as a cooperate game between the rationale generator (\aka data augmentation module in SimCLR) and the contrastive learner making use of only the discovered rationales.
The two players aim for the shared goal of achieving semantically-good representations, just having to operate within the confines imposed by rationale discovery.

Formally, our goal is to generate a rationale, denoted as $R(\Mat{g})$, which is a selection of nodes or subgraphs in $\Mat{g}$ that accounts for self-discrimination.
An ideal rationale should satisfy the sufficiency condition --- $R(\Mat{g})$ is sufficient to preserve the critical information of $\Mat{g}$ and generate the semantically good representation:
\begin{gather}
    f(R(\Mat{g}))=f(\Mat{g}),
\end{gather}
Moreover, according to the comprehensiveness condition, the complement of rationale does 

There are two justifications of the comprehensiveness condition.
First, it regulates the information outside the rationale, so that the rationale contains all the relevant and useful information.
Second and more importantly, comprehensiveness is promising to prevent the explanations from degeneration, where the $R(\Mat{g})$ attempts to encode the self-discrimination of $\Mat{g}$ using trivial information.

\wx{To fit the comprehensiveness condition, can we set the complement $C(\Mat{g})=\Mat{g}\setminus R(\Mat{g})$ as the negative view of the anchor graph $\Mat{g}$?
\begin{gather}
    f(g)\perp C(g) | R(g),
\end{gather}


\section{Methodology}
\subsection{Rationale Discovery}
\begin{gather}
    \Mat{Z} = \text{GNN}(g),
\end{gather}

\begin{gather}
    p(\Mat{M}|\Mat{Z}) = \Pi_{v\in\Set{V}}p(v|\Mat{z})
\end{gather}

We can try the reparameterization trick to generate the rationale mask:
\begin{gather}
    p(v|\Mat{z}) = \sigma((\log{\frac{\epsilon}{1-\epsilon}}+\alpha)),\quad\alpha=\text{MLP}(\Mat{z}),
\end{gather}
or directly use:
\begin{gather}
    p(v|\Mat{z}) = \text{MLP}(\Mat{z}),
\end{gather}

\begin{gather}
    R(g)\sim p(\Mat{M}|\Mat{Z})
\end{gather}


\subsection{Representation Learning}

The GNN encoder $f(\cdot)$ extracts representations from the augmented graphs, including rationales and complements.
The projection head $h(\cdot)$ maps representations to the space where contrastive loss is applied.
Formally, the representation and projection of the rationale $R(g)$ are:
\begin{gather}
    \Mat{r} = f(R(g)),\quad\Mat{a}=h(\Mat{r}),
\end{gather}
where $\Mat{a}$ is $L_{2}$ normalized.
Similarly, the representation and projection of the complement $C(g)$ are:
\begin{gather}
    \Mat{c}=f(C(g)),\quad\Mat{b}=h(\Mat{c}),
\end{gather}
where $\Mat{b}$ is $L_{2}$ normalized.



\subsection{Pre-Training Scheme}
We randomly sample a minibatch of $N$ graph instances and define the contrastive prediction task on pairs of augmented graphs derived from the minibatch, resulting in $2N$ rationales and $2N$ complements.
Given a positive rationale pair, we treat the other $2(N-1)$ rationales and $2N$ complements within a minibatch as negative examples.


% The loss function for a positive pair of rationales $(r_{i},r_{j})$ is defined as:
% \begin{align}
%     l(r_{i},r_{j})=&-\log{\frac{\exp{s(r_{i},r_{j})/\tau}}{\sum_{k=1}^{2N}\Space{I}_{k\neq i}\exp{s(r_{i},r_{k})/\tau}}}\nonumber\\
%     &-\log{\frac{\exp{s(r_{i},r_{j})/\tau}}{\sum_{k=1}^{2N}\exp{s(r_{i},c_{k})/\tau}}}
% \end{align}

The loss function for a positive pair of rationales $(r_{i},r_{j})$ is defined as:
\begin{align}
    l(r_{i},r_{j})=&-\log{\frac{\exp{(\Trans{\Mat{a}}_{i}\Mat{a}_{j}/\tau)}}{\sum_{k=1}^{2N}\Space{I}_{k\neq i}\exp{(\Trans{\Mat{a}}_{i}\Mat{a}_{k}/\tau)}}}\nonumber\\
    &-\log{\frac{\exp{(\Trans{\Mat{a}}_{i}\Mat{a}_{j}/\tau)}}{\sum_{k=1}^{2N}\exp{(\Trans{\Mat{a}}_{i}\Mat{b}_{k}/\tau)}}},
\end{align}
where $\Space{I}_{k\neq i}\in\{0,1\}$ is an indicator function evaluating to $1$ iff $k\neq i$ and $\tau$ denotes a temperature parameter.
Within the loss, the first term encourages the sufficient condition (\ie the rationale $R(g)$ is sufficient to preserve the critical information of $g$), while the second term enforces the comprehensiveness condition (\ie the complement $C(g)$ regulates the information outside the rationale).
Or, we can try another version as follows:
\begin{align}
    &l(r_{i},r_{j})=\\
    &-\log{\frac{\exp{(\Trans{\Mat{a}}_{i}\Mat{a}_{j}/\tau)}}{\sum_{k=1}^{2N}\Space{I}_{k\neq i}\exp{(\Trans{\Mat{a}}_{i}\Mat{a}_{k}/\tau)}+\exp{(\Trans{\Mat{a}}_{i}\Mat{b}_{k}/\tau)}}}.\nonumber
\end{align}




}
